Investigating the Compton amplitude subtraction function in lattice QCD

Theoretical predictions of the proton--neutron mass difference and measurements of the proton's charge radius require inputs from the Compton amplitude subtraction function. Model-dependent and non-relativistic calculations of this subtraction function vary significantly, and hence it contributes sizeable uncertainties to the aforementioned physical quantities. We report on the use of Feynman-Hellmann methods in lattice QCD to calculate the subtraction function from first principles. In particular, our initial results show anomalous high-energy behaviour that is at odds with the prediction from the operator product expansion (OPE). Therefore, we investigate the possibility that this unexpected behaviour is due to lattice artifacts, by varying the lattice spacing and volume, and comparing different discretisations of the vector current. Finally, we explore a Feynman-Hellmann implementation that is less sensitive to short-distance contributions and show that the subtraction function's anomalous behaviour can be attributed to these short-distance contributions. As such, this work represents the first steps in achieving a complete understanding of the Compton amplitude subtraction function.

==> fig-interlacing.tex <==
 \begin{figure}
 
\centering

%%%%%%%%%%%%%%%%%%% ALL T SLICES %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{0.27\linewidth}

\centering
{
\begin{tikzpicture}[scale=0.6]
\def\max{8}
\def\z{0.75}

% The axes
\draw[help lines,->] (0,0) -- (\max*\z,0) coordinate (xaxis);
\draw[help lines,->] (0,0) -- (0,\max*\z) coordinate (yaxis);

\draw[step=\z,gray,line width = 0.01mm] (0,0) grid (\max*\z,\max*\z);
    
 \foreach \x in {0,1,...,\max}{% Two indices running over each
   %   \foreach \y in {1,...,\max}{% node on the grid we have drawn 
       \foreach \y in {\x,...,\max}{% node on the grid we have drawn 
        \node[draw,circle,inner sep=2.5,fill=blue] at (\x*\z,\y*\z) {};
            % Places a dot at those points
      }
    }

\draw[yellow, line width = 0.7mm] (0,0) -- (\max*\z,\max*\z);

% The labels
\node[below] at (xaxis) {$t_1$};
\node[above] at (yaxis) {$t_2$};

\end{tikzpicture}}
\caption{No interlacing ($\tmin=0$).}
\label{fig:interlacing.a}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\centering
{
\begin{tikzpicture}[scale=0.6]
\def\max{8}
\def\halfmax{4}
\def\z{0.75}

% The axes
\draw[help lines,->] (0,0) -- (\max*\z,0) coordinate (xaxis);
\draw[help lines,->] (0,0) -- (0,\max*\z) coordinate (yaxis);

\draw[step=\z,gray,line width = 0.01mm] (0,0) grid (\max*\z,\max*\z);
 \foreach \x in {1,2,...,\halfmax}{% Two indices running over each
      \foreach \y in {\x,...,\halfmax}{% node on the grid we have drawn 
        \node[draw,circle,inner sep=2.5,fill=blue] at (\x*2*\z-2*\z,\y*2*\z-\z) {};
            % Places a dot at those points
      }
    }
    
 \foreach \x in {1,2,...,\halfmax}{% Two indices running over each
      \foreach \y in {\x,...,\halfmax}{% node on the grid we have drawn 
        \node[draw,circle,inner sep=2.5,fill=blue] at (\x*2*\z-\z,\y*2*\z) {};
            % Places a dot at those points
      }
    }
 
% The axes

\draw[yellow, line width = 0.7mm] (0,0) -- (\max*\z,\max*\z);
 


% The labels
\node[below] at (xaxis) {$t_1$};
\node[above] at (yaxis) {$t_2$};

\end{tikzpicture}}
\caption{Interlacing $\tmin=1$.}
\label{fig:interlacing.b}
\end{subfigure}
\begin{subfigure}{0.25\linewidth}
\centering
{
\begin{tikzpicture}[scale=0.6]
\def\z{0.75}
\def\max{8}
\def\hal\max{4}

% The axes
\draw[help lines,->] (0,0) -- (\max*\z,0) coordinate (xaxis);
\draw[help lines,->] (0,0) -- (0,\max*\z) coordinate (yaxis);

\draw[step=\z,gray,line width = 0.01mm] (0,0) grid (\max*\z,\max*\z);
 \foreach \x in {1,2}{% Two indices running over each
      \foreach \y in {\x,...,2}{% node on the grid we have drawn 
        \node[draw,circle,inner sep=2.5,fill=blue] at (\x*4*\z-4*\z,\y*4*\z-2*\z) {};
            % Places a dot at those points
      }
    }
    
 \foreach \x in {1,2}{% Two indices running over each
      \foreach \y in {\x,...,2}{% node on the grid we have drawn 
        \node[draw,circle,inner sep=2.5,fill=blue] at (\x*4*\z-2*\z,\y*4*\z) {};
            % Places a dot at those points
      }
    }    
 
 

\draw[yellow, line width = 0.7mm] (0,0) -- (\max*\z,\max*\z);

% The labels
\node[below] at (xaxis) {$t_1$};
\node[above] at (yaxis) {$t_2$};

\end{tikzpicture}}
\caption{Interlacing $\tmin=2$.}
\label{fig:interlacing.c}
\end{subfigure}
\caption{Integration regions for different temporal interlacings, with the time-ordering $t_2\geq t_1$. The blue dots represent pairs of time slices with current insertions, while the yellow line is the $t_1=t_2$ line. }
\label{fig:interlacing}
\end{figure}

